Limitations of Mean-Based Algorithms for Trace Reconstruction at Small Distance

Trace reconstruction considers the task of recovering an unknown string $x \in \{0,1\}^n$ given a number of independent "traces", i.e., subsequences of $x$ obtained by randomly and independently deleting every symbol of $x$ with some probability $p$. The information-theoretic limit of the number of traces needed to recover a string of length $n$ is still unknown. This limit is essentially the same as the number of traces needed to determine, given strings $x$ and $y$ and traces of one of them, which string is the source. The most-studied class of algorithms for the worst-case version of the problem are "mean-based" algorithms. These are a restricted class of distinguishers that only use the mean value of each coordinate on the given samples. In this work we study limitations of mean-based algorithms on strings at small Hamming or edit distance. We show that, on the one hand, distinguishing strings that are nearby in Hamming distance is "easy" for such distinguishers. On the other hand, we show that distinguishing strings that are nearby in edit distance is "hard" for mean-based algorithms. Along the way, we also describe a connection to the famous Prouhet-Tarry-Escott (PTE) problem, which shows a barrier to finding explicit hard-to-distinguish strings: namely such strings would imply explicit short solutions to the PTE problem, a well-known difficult problem in number theory. Furthermore, we show that the converse is also true, thus, finding explicit solutions to the PTE problem is equivalent to the problem of finding explicit strings that are hard-to-distinguish by mean-based algorithms. Our techniques rely on complex analysis arguments that involve careful trigonometric estimates, and algebraic techniques that include applications of Descartes' rule of signs for polynomials over the reals.

==> smallEdit.tex <==
\section{Hard strings at edit distance 4} \label{sec:edist-four}
The goal of this section is to prove Theorem~\ref{thm:main-edist-four}, and thus exhibit two strings at edit distance $4$ such that every mean-based algorithm requires super-polynomially many traces.


Before proving Theorem~\ref{thm:main-edist-four}, we need the following lemma about estimation of trigonometric functions.
\begin{lemma} \label{lem:trig-estimates}
The following bounds hold:
\begin{enumerate}
\item
For integer $d \ge 1$ and $\varphi$ such that $\abs{d\varphi} \le \frac{\pi}{3}$, we have $\cos\tp{d\varphi} \le \tp{\cos\varphi}^d$.
\item
Let integer $d \ge 1$ and $\theta$ be such that $\abs{d\cdot\frac{\theta}{2}} < \frac{\pi}{3}$. Let $w=\tp{1+e^{i\theta}}/2$. Then $\abs{w^d-1} < 2\abs{\sin\tp{\frac{d\theta}{4}}}$.
\end{enumerate}
\end{lemma}
\begin{proof}
\begin{enumerate}
\item 
The inequality is trivially true when $d=1$. We also have 
\begin{align*}
\cos\tp{(d+1)\varphi} = \cos\tp{d\varphi}\cos\varphi - \sin\tp{d\varphi}\sin\varphi \le \cos\tp{d\varphi}\cos\varphi. 
\end{align*}
The inequality is due to $\sin(d\varphi)\sin\varphi \ge 0$. Therefore an induction on $d$ finishes the proof.
\item
We can write 
\begin{align*}
w = \frac{1+\cos\theta}{2} + i \cdot \frac{\sin\theta}{2} = \cos\frac{\theta}{2}\tp{\cos\frac{\theta}{2} + i\sin\frac{\theta}{2}}, 
\end{align*}
and
\begin{align*}
w^d = \tp{\cos\frac{\theta}{2}}^d \cdot \tp{\cos\frac{d\theta}{2} + i\sin\frac{d\theta}{2}}. 
\end{align*}
Therefore
\begin{align*}
\abs{w^d-1}^2 &= \tp{\tp{\cos\frac{\theta}{2}}^d \cdot \cos\frac{d\theta}{2} - 1}^2 + \tp{\tp{\cos\frac{\theta}{2}}^d \cdot \sin\frac{d\theta}{2}}^2 \\
&= \tp{\cos\frac{\theta}{2}}^{2d}-2\tp{\cos\frac{\theta}{2}}^d\cos\frac{d\theta}{2}+1 \\
&= \tp{\tp{\cos\frac{\theta}{2}}^d - \cos\frac{d\theta}{2}}^2 + \tp{\sin\frac{d\theta}{2}}^2.
\end{align*}
By item (1), $\cos\tp{d\theta/2} \le \cos^d\tp{\theta/2}$ and hence 
\begin{align*}
\abs{w^d-1}^2 \le \tp{1 - \cos\frac{d\theta}{2}}^2 + \tp{\sin\frac{d\theta}{2}}^2 = 2 - 2\cos\frac{d\theta}{2} = 4\tp{\sin\frac{d\theta}{4}}^2,
\end{align*}
which implies $\abs{w^d-1} \le 2\abs{\sin\frac{d\theta}{4}}$.
\end{enumerate}
\end{proof}

We will prove the following theorem, which is a more concrete version of Theorem~\ref{thm:main-edist-four}.

\begin{theorem} \label{thm:concrete-edist-four}
Assume the deletion probability $p=1/2$. Let $k$ be an odd integer and $n=\sum_{j=0}^{k}3^j$ be an even integer, and $R(w)=\prod_{j=0}^{k}\tp{1-w^{3^j}}$ be a polynomial of degree $n$. Let $E_n(w) = \sum_{j=0}^{n/2}w^{2j}$. Then $Q_{\*e}(w) \coloneqq R(w) + E_n(w)$ is a 0/1-coefficient polynomial which corresponds to a string $\*e \in \set{0, 1}^n$. Moreover, any two strings $\*x$, $\*y$ of the form $\*x=\*a10\*e$ and $\*y=\*a\*e01$ satisfy
\begin{align*}
    \sup\set{\abs{Q_{\*x}(w) - Q_{\*y}(w)} \colon w \in \partial B(p;q)} \le \exp\tp{-\Omega(\log^2 n)},
\end{align*}
where $\*a$ is an arbitrary string of length $n$.
\end{theorem}
\begin{proof}
$R(w)$ has the following properties: (1) The coefficients of $R$ belong to $\set{-1,0,1}$ since each monomial occurs only once in the expansion. (2) Odd-degree terms have negative signs, and even-degree terms have positive signs. It follows that $R(w) + E_n(w)$ is a polynomial with 0/1 coefficients. 

We can write 
\begin{align*}
P(w) &= Q_{\*x}(w) - Q_{\*y}(w) = w^n\tp{(w^2-1)Q_{\*e}(w) - \tp{w^{n+2}-1}} \\
&= w^n(w^2-1)\tp{Q_{\*e}(w) - E_n(w)} \\
&= w^n(w^2-1)R(w).
\end{align*}

Consider a point $w=\tp{1+e^{i\theta}}/2$ on the circle $\partial B(1/2; 1/2)$, where $\theta \in [-\pi, \pi]$. We consider two cases.
\begin{enumerate}
    \item $|\theta/2| \ge 3^{-k/4}\pi$. Using the bound $|\cos x| \le 1 - (2x/\pi)^2$ for $|x| \le \pi/2$, we have in this case $|w| = \abs{\cos\frac{\theta}{2}} \le 1-4\cdot 3^{-k/2}$, and
    \begin{align*}
        |P(w)| \le |w|^n \cdot 2(n+1) \le \tp{1 - 4\cdot 3^{-k/2}}^n \cdot 2(n+1) \le \exp\tp{-\Omega\tp{\sqrt{n}}}.
    \end{align*}
    The last inequality is because $1-x < e^{-x}$ and $n=\sum_{j=0}^{k}3^j < 3^{k+1}$.
    \item $|\theta/2| < 3^{-k/4}\pi$. Note that when $j \le k/4-1$, $|3^j \cdot \frac{\theta}{2}| < \frac{\pi}{3}$. Therefore by item (2) of Lemma~\ref{lem:trig-estimates}, we have $|w^{3^j}-1| \le 2\abs{\sin\tp{3^j\theta/4}}$. Using the fact that $|\sin x| \le |x|$, we have
    \begin{align*}
        |R(w)| &\le \prod_{j=0}^{k/4-1}\abs{w^{3^j}-1} \cdot \prod_{j=k/4}^{k}\abs{w^{3^j}-1} \le \prod_{j=0}^{k/4-1} \abs{\frac{3^j\theta}{2}} \cdot 2^{3k/4} \le \prod_{j=1}^{k/4}\tp{3^{-j}\pi} \cdot 2^{3k/4} \\
        &\le \exp\tp{-\Omega(k^2)} \cdot \exp\tp{O(k)} = \exp\tp{-\Omega(k^2)} = \exp\tp{-\Omega\tp{\log^2 n}}.
    \end{align*}
    Therefore $|P(w)| \le 2|R(w)| \le \exp\tp{-\Omega\tp{\log^2 n}}$.
\end{enumerate}
\end{proof}

The edit distance between strings $\*x$ and $\*y$ constructed in the theorem above is clearly at most 4. Thus, Theorem~\ref{thm:main-edist-four} follows via Theorem~\ref{thm:reduction-to-comp} (see Appendix~\ref{sec:reduction} for its proof).

\enote{TODO}
\begin{corollary}(PTE solutions)\label{cor:exp-pte-sols}
For $\*x$ and $\*y$ obtained from Theorem~\ref{thm:main-edist-four} with $\*a={\bf 0}$,  consider the set  $A=\{i\mid \*x_i\ne 0\}$ and $B=\{i\mid \*y_i\ne 0\}.$  Then the sets $A$ and $B$ form a solution to the PTE problem with size $s=2^{k'-1}$ and degree $k=(k+1)3^k????$.
\end{corollary}


